Sparse Inverse Covariance Estimation via an Adaptive Gradient-Based Method

We study the problem of estimating from data, a sparse approximation to the inverse covariance matrix. Estimating a sparsity constrained inverse covariance matrix is a key component in Gaussian graphical model learning, but one that is numerically very challenging. We address this challenge by developing a new adaptive gradient-based method that carefully combines gradient information with an adaptive step-scaling strategy, which results in a scalable, highly competitive method. Our algorithm, like its predecessors, maximizes an $\ell_1$-norm penalized log-likelihood and has the same per iteration arithmetic complexity as the best methods in its class. Our experiments reveal that our approach outperforms state-of-the-art competitors, often significantly so, for large problems.

==> header.tex <==
\RequirePackage{amsfonts}
\RequirePackage{amsmath}
\RequirePackage{bm}
\RequirePackage{mathrsfs}

% ================= OVERALL DEFS ======================
\newcommand{\bmt}[1]{\bm{#1}^T}

% %%%%%%%%%%%%%  VECTORS %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\va}{\bm{a}}       \newcommand{\vah}{\hat{\bm{a}}}        \newcommand{\ah}{\hat{a}}    \newcommand{\vat}{\tilde{\bm{a}}}       \newcommand{\at}{\tilde{a}}
\newcommand{\vb}{\bm{b}}       \newcommand{\vbh}{\hat{\bm{b}}}        \newcommand{\bh}{\hat{b}}    \newcommand{\vbt}{\tilde{\bm{b}}}       \newcommand{\bt}{\tilde{b}}
\newcommand{\vc}{\bm{c}}       \newcommand{\vch}{\hat{\bm{c}}}        \newcommand{\ch}{\hat{c}}    \newcommand{\vct}{\tilde{\bm{c}}}       \newcommand{\ct}{\tilde{c}}
\newcommand{\vd}{\bm{d}}       \newcommand{\vdh}{\hat{\bm{d}}}        \newcommand{\dhat}{\hat{d}}  \newcommand{\vdt}{\tilde{\bm{d}}}       \newcommand{\dt}{\tilde{d}}
\newcommand{\ve}{\bm{e}}       \newcommand{\veh}{\hat{\bm{e}}}        \newcommand{\eh}{\hat{e}}    \newcommand{\vet}{\tilde{\bm{e}}}       \newcommand{\et}{\tilde{e}}
\newcommand{\vf}{\bm{f}}       \newcommand{\vfh}{\hat{\bm{f}}}        \newcommand{\fh}{\hat{f}}    \newcommand{\vft}{\tilde{\bm{f}}}       \newcommand{\ft}{\tilde{f}}
\newcommand{\vg}{\bm{g}}       \newcommand{\vgh}{\hat{\bm{g}}}        \newcommand{\gh}{\hat{g}}    \newcommand{\vgt}{\tilde{\bm{g}}}       \newcommand{\gt}{\tilde{g}}
\newcommand{\vech}{\bm{h}}     \newcommand{\vhh}{\hat{\bm{h}}}        \newcommand{\hh}{\hat{h}}    \newcommand{\vht}{\tilde{\bm{h}}}       \newcommand{\htild}{\tilde{h}}
\newcommand{\vi}{\bm{i}}       \newcommand{\vih}{\hat{\bm{i}}}        \newcommand{\ih}{\hat{i}}    \newcommand{\vit}{\tilde{\bm{i}}}       \newcommand{\itild}{\tilde{i}}
\newcommand{\vj}{\bm{j}}       \newcommand{\vjh}{\hat{\bm{j}}}        \newcommand{\jh}{\hat{j}}    \newcommand{\vjt}{\tilde{\bm{j}}}       \newcommand{\jt}{\tilde{j}}
\newcommand{\vk}{\bm{k}}       \newcommand{\vkh}{\hat{\bm{k}}}        \newcommand{\kh}{\hat{k}}    \newcommand{\vkt}{\tilde{\bm{k}}}       \newcommand{\kt}{\tilde{k}}
\newcommand{\vl}{\bm{l}}       \newcommand{\vlh}{\hat{\bm{l}}}        \newcommand{\lh}{\hat{l}}    \newcommand{\vlt}{\tilde{\bm{l}}}       \newcommand{\lt}{\tilde{l}}
\newcommand{\vm}{\bm{m}}       \newcommand{\vmh}{\hat{\bm{m}}}        \newcommand{\mh}{\hat{m}}    \newcommand{\vmt}{\tilde{\bm{m}}}       \newcommand{\mt}{\tilde{m}}
\newcommand{\vn}{\bm{n}}       \newcommand{\vnh}{\hat{\bm{n}}}        \newcommand{\nh}{\hat{n}}    \newcommand{\vnt}{\tilde{\bm{n}}}       \newcommand{\nt}{\tilde{n}}
\newcommand{\vo}{\bm{o}}       \newcommand{\voh}{\hat{\bm{o}}}        \newcommand{\oh}{\hat{o}}    \newcommand{\vot}{\tilde{\bm{o}}}       \newcommand{\ot}{\tilde{o}}
\newcommand{\vp}{\bm{p}}       \newcommand{\vph}{\hat{\bm{p}}}        \newcommand{\ph}{\hat{p}}    \newcommand{\vpt}{\tilde{\bm{p}}}       \newcommand{\pt}{\tilde{p}}
\newcommand{\vq}{\bm{q}}       \newcommand{\vqh}{\hat{\bm{q}}}        \newcommand{\qh}{\hat{q}}    \newcommand{\vqt}{\tilde{\bm{q}}}       \newcommand{\qt}{\tilde{q}}
\newcommand{\vr}{\bm{r}}       \newcommand{\vrh}{\hat{\bm{r}}}        \newcommand{\rh}{\hat{r}}    \newcommand{\vrt}{\tilde{\bm{r}}}       \newcommand{\rt}{\tilde{r}}
\newcommand{\vs}{\bm{s}}       \newcommand{\vsh}{\hat{\bm{s}}}        \newcommand{\sh}{\hat{s}}    \newcommand{\vst}{\tilde{\bm{s}}}       \newcommand{\st}{\tilde{s}}
\newcommand{\vt}{\bm{t}}       \newcommand{\vth}{\hat{\bm{t}}}        \newcommand{\that}{\hat{t}}  \newcommand{\vtt}{\tilde{\bm{t}}}       \newcommand{\ttil}{\tilde{t}}
\newcommand{\vu}{\bm{u}}       \newcommand{\vuh}{\hat{\bm{u}}}        \newcommand{\uh}{\hat{u}}    \newcommand{\vut}{\tilde{\bm{u}}}       \newcommand{\ut}{\tilde{u}}
\newcommand{\vv}{\bm{v}}       \newcommand{\vvh}{\hat{\bm{v}}}        \newcommand{\vh}{\hat{v}}    \newcommand{\vvt}{\tilde{\bm{v}}}       \newcommand{\vtild}{\tilde{v}}
\newcommand{\vw}{\bm{w}}       \newcommand{\vwh}{\hat{\bm{w}}}        \newcommand{\wh}{\hat{w}}    \newcommand{\vwt}{\tilde{\bm{w}}}       \newcommand{\wt}{\tilde{w}}
\newcommand{\vx}{\bm{x}}       \newcommand{\vxh}{\hat{\bm{x}}}        \newcommand{\xh}{\hat{x}}    \newcommand{\vxt}{\tilde{\bm{x}}}       \newcommand{\xt}{\tilde{x}}
\newcommand{\vy}{\bm{y}}       \newcommand{\vyh}{\hat{\bm{y}}}        \newcommand{\yh}{\hat{y}}    \newcommand{\vyt}{\tilde{\bm{y}}}       \newcommand{\yt}{\tilde{y}}
\newcommand{\vz}{\bm{z}}       \newcommand{\vzh}{\hat{\bm{z}}}        \newcommand{\zh}{\hat{z}}    \newcommand{\vzt}{\tilde{\bm{z}}}       \newcommand{\zt}{\tilde{z}}

% %%%%%%%%%%%%%%%%%%%% BOLD GREEK %%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\valpha}  {\bm{\alpha}}      \newcommand{\valphah}  {\hat{\bm{\alpha}}}       \newcommand{\valphat}  {\tilde{\bm{\alpha}}}       \newcommand{\alphat}  {\tilde{\alpha}}
\newcommand{\vbeta}   {\bm{\beta}}       \newcommand{\vbetah}   {\hat{\bm{\beta}}}        \newcommand{\vbetat}   {\tilde{\bm{\beta}}}        \newcommand{\betat}   {\tilde{\beta}}
\newcommand{\vdelta}  {\bm{\delta}}      \newcommand{\vdeltah}  {\hat{\bm{\delta}}}       \newcommand{\vdeltat}  {\tilde{\bm{\delta}}}       \newcommand{\deltat}  {\tilde{\delta}}
\newcommand{\vepsilon}{\bm{\epsilon}}    \newcommand{\vepsilonh}{\hat{\bm{\epsilon}}}     \newcommand{\vepsilont}{\tilde{\bm{\epsilon}}}     \newcommand{\epsilont}{\tilde{\epsilon}}
\newcommand{\vphi}    {\bm{\phi}}        \newcommand{\vphih}    {\hat{\bm{\phi}}}         \newcommand{\vphit}    {\tilde{\bm{\phi}}}         \newcommand{\phit}    {\tilde{\phi}}
\newcommand{\vgamma}  {\bm{\gamma}}      \newcommand{\vgammah}  {\hat{\bm{\gamma}}}       \newcommand{\vgammat}  {\tilde{\bm{\gamma}}}       \newcommand{\gammat}  {\tilde{\gamma}}
\newcommand{\veta}    {\bm{\eta}}        \newcommand{\vetah}    {\hat{\bm{\eta}}}         \newcommand{\vetat}    {\tilde{\bm{\eta}}}         \newcommand{\etat}    {\tilde{\eta}}
\newcommand{\vtheta}  {\bm{\theta}}      \newcommand{\vthetah}  {\hat{\bm{\theta}}}       \newcommand{\vthetat}  {\tilde{\bm{\theta}}}       \newcommand{\thetat}  {\tilde{\theta}}
\newcommand{\vkappa}  {\bm{\kappa}}      \newcommand{\vkappah}  {\hat{\bm{\kappa}}}       \newcommand{\vkappat}  {\tilde{\bm{\kappa}}}       \newcommand{\kappat}  {\tilde{\kappa}}
\newcommand{\vlambda} {\bm{\lambda}}     \newcommand{\vlambdah} {\hat{\bm{\lambda}}}      \newcommand{\vlambdat} {\tilde{\bm{\lambda}}}      \newcommand{\lambdat} {\tilde{\lambda}}
\newcommand{\vmu}     {\bm{\mu}}         \newcommand{\vmuh}     {\hat{\bm{\mu}}}          \newcommand{\vmut}     {\tilde{\bm{\mu}}}          \newcommand{\mut}     {\tilde{\mu}}
\newcommand{\vnu}     {\bm{\nu}}         \newcommand{\vnuh}     {\hat{\bm{\nu}}}          \newcommand{\vnut}     {\tilde{\bm{\nu}}}          \newcommand{\nut}     {\tilde{\nu}}
\newcommand{\vpi}     {\bm{\pi}}         \newcommand{\vpih}     {\hat{\bm{\pi}}}          \newcommand{\vpit}     {\tilde{\bm{\pi}}}          \newcommand{\pit}     {\tilde{\pi}}
\newcommand{\vchi}    {\bm{\chi}}        \newcommand{\vchih}    {\hat{\bm{\chi}}}         \newcommand{\vchit}    {\tilde{\bm{\chi}}}         \newcommand{\chit}    {\tilde{\chi}}
\newcommand{\vrho}    {\bm{\rho}}        \newcommand{\vrhoh}    {\hat{\bm{\rho}}}         \newcommand{\vrhot}    {\tilde{\bm{\rho}}}         \newcommand{\rhot}    {\tilde{\rho}}
\newcommand{\vsigma}  {\bm{\sigma}}      \newcommand{\vsigmah}  {\hat{\bm{\sigma}}}       \newcommand{\vsigmat}  {\tilde{\bm{\sigma}}}       \newcommand{\sigmat}  {\tilde{\sigma}}
\newcommand{\vtau}    {\bm{\tau}}        \newcommand{\vtauh}    {\hat{\bm{\tau}}}         \newcommand{\vtaut}    {\tilde{\bm{\tau}}}         \newcommand{\taut}    {\tilde{\tau}}
\newcommand{\vupsilon}{\bm{\upsilon}}    \newcommand{\vupsilonh}{\hat{\bm{\upsilon}}}     \newcommand{\vupsilont}{\tilde{\bm{\upsilon}}}     \newcommand{\upsilont}{\tilde{\upsilon}}
\newcommand{\vomega}  {\bm{\omega}}      \newcommand{\vomegah}  {\hat{\bm{\omega}}}       \newcommand{\vomegat}  {\tilde{\bm{\omega}}}       \newcommand{\omegat}  {\tilde{\omega}}
\newcommand{\vxi}     {\bm{\xi}}         \newcommand{\vxih}     {\hat{\bm{\xi}}}          \newcommand{\vxit}     {\tilde{\bm{\xi}}}          \newcommand{\xit}     {\tilde{\xi}}
\newcommand{\vpsi}    {\bm{\psi}}        \newcommand{\vpsih}    {\hat{\bm{\psi}}}         \newcommand{\vpsit}    {\tilde{\bm{\psi}}}         \newcommand{\psit}    {\tilde{\psi}}
\newcommand{\vzeta}   {\bm{\zeta}}       \newcommand{\vzetah}   {\hat{\bm{\zeta}}}        \newcommand{\vzetat}   {\tilde{\bm{\zeta}}}        \newcommand{\zetat}   {\tilde{\zeta}}


% %%%%%%%%%%%%%  MATRICES %%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\ma}{\bm{A}}       \newcommand{\mah}{\hat{\bm{A}}}        \newcommand{\mawh}{\widehat{\bm{A}}} \newcommand{\mat}{\tilde{\bm{A}}}        \newcommand{\mawt}{\widetilde{\bm{A}}}
\newcommand{\mb}{\bm{B}}       \newcommand{\mbh}{\hat{\bm{B}}}        \newcommand{\mbwh}{\widehat{\bm{B}}} \newcommand{\mbt}{\tilde{\bm{B}}}        \newcommand{\mbwt}{\widetilde{\bm{B}}}
\newcommand{\mc}{\bm{C}}       \newcommand{\mch}{\hat{\bm{C}}}        \newcommand{\mcwh}{\widehat{\bm{C}}} \newcommand{\mct}{\tilde{\bm{C}}}        \newcommand{\mcwt}{\widetilde{\bm{C}}}
\newcommand{\md}{\bm{D}}       \newcommand{\mdh}{\hat{\bm{D}}}        \newcommand{\mdwh}{\widehat{\bm{D}}} \newcommand{\mdt}{\tilde{\bm{D}}}        \newcommand{\mdwt}{\widetilde{\bm{D}}}
\newcommand{\me}{\bm{E}}       \newcommand{\meh}{\hat{\bm{E}}}        \newcommand{\mewh}{\widehat{\bm{E}}} \newcommand{\met}{\tilde{\bm{E}}}        \newcommand{\mewt}{\widetilde{\bm{E}}}
\newcommand{\mf}{\bm{F}}       \newcommand{\mfh}{\hat{\bm{F}}}        \newcommand{\mfwh}{\widehat{\bm{F}}} \newcommand{\mft}{\tilde{\bm{F}}}        \newcommand{\mfwt}{\widetilde{\bm{F}}}
\newcommand{\mg}{\bm{G}}       \newcommand{\mgh}{\hat{\bm{G}}}        \newcommand{\mgwh}{\widehat{\bm{G}}} \newcommand{\mgt}{\tilde{\bm{G}}}        \newcommand{\mgwt}{\widetilde{\bm{G}}}
\newcommand{\mH}{\bm{H}}       \newcommand{\mhh}{\hat{\bm{H}}}        \newcommand{\mhwh}{\widehat{\bm{H}}} \newcommand{\mht}{\tilde{\bm{H}}}        \newcommand{\mhwt}{\widetilde{\bm{H}}}
\newcommand{\mi}{\bm{I}}       \newcommand{\mih}{\hat{\bm{I}}}        \newcommand{\miwh}{\widehat{\bm{I}}} \renewcommand{\mit}{\tilde{\bm{I}}}      \newcommand{\miwt}{\widetilde{\bm{I}}}
\newcommand{\mj}{\bm{J}}       \newcommand{\mjh}{\hat{\bm{J}}}        \newcommand{\mjwh}{\widehat{\bm{J}}} \newcommand{\mjt}{\tilde{\bm{J}}}        \newcommand{\mjwt}{\widetilde{\bm{J}}}
\newcommand{\mk}{\bm{K}}       \newcommand{\mkh}{\hat{\bm{K}}}        \newcommand{\mkwh}{\widehat{\bm{K}}} \newcommand{\mkt}{\tilde{\bm{K}}}        \newcommand{\mkwt}{\widetilde{\bm{K}}}
\newcommand{\ml}{\bm{L}}       \newcommand{\mlh}{\hat{\bm{L}}}        \newcommand{\mlwh}{\widehat{\bm{L}}} \newcommand{\mlt}{\tilde{\bm{L}}}        \newcommand{\mlwt}{\widetilde{\bm{L}}}
\newcommand{\mm}{\bm{M}}       \newcommand{\mmh}{\hat{\bm{M}}}        \newcommand{\mmwh}{\widehat{\bm{M}}} \newcommand{\mmt}{\tilde{\bm{M}}}        \newcommand{\mmwt}{\widetilde{\bm{M}}}
\newcommand{\mn}{\bm{N}}       \newcommand{\mnh}{\hat{\bm{N}}}        \newcommand{\mnwh}{\widehat{\bm{N}}} \newcommand{\mnt}{\tilde{\bm{N}}}        \newcommand{\mnwt}{\widetilde{\bm{N}}}
\newcommand{\mo}{\bm{O}}       \newcommand{\moh}{\hat{\bm{O}}}        \newcommand{\mowh}{\widehat{\bm{O}}} \newcommand{\mot}{\tilde{\bm{O}}}        \newcommand{\mowt}{\widetilde{\bm{O}}}
\newcommand{\mP}{\bm{P}}       \newcommand{\mph}{\hat{\bm{P}}}        \newcommand{\mpwh}{\widehat{\bm{P}}} \newcommand{\mpt}{\tilde{\bm{P}}}        \newcommand{\mpwt}{\widetilde{\bm{P}}}
\newcommand{\mq}{\bm{Q}}       \newcommand{\mqh}{\hat{\bm{Q}}}        \newcommand{\mqwh}{\widehat{\bm{Q}}} \newcommand{\mqt}{\tilde{\bm{Q}}}        \newcommand{\mqwt}{\widetilde{\bm{Q}}}
\newcommand{\mr}{\bm{R}}       \newcommand{\mrh}{\hat{\bm{R}}}        \newcommand{\mrwh}{\widehat{\bm{R}}} \newcommand{\mrt}{\tilde{\bm{R}}}        \newcommand{\mrwt}{\widetilde{\bm{R}}}
\newcommand{\ms}{\bm{S}}       \newcommand{\msh}{\hat{\bm{S}}}        \newcommand{\mswh}{\widehat{\bm{S}}} \newcommand{\mst}{\tilde{\bm{S}}}        \newcommand{\mswt}{\widetilde{\bm{S}}}
\newcommand{\mT}{\bm{T}}       \newcommand{\mth}{\hat{\bm{T}}}        \newcommand{\mtwh}{\widehat{\bm{T}}} \newcommand{\mtt}{\tilde{\bm{T}}}        \newcommand{\mtwt}{\widetilde{\bm{T}}}
\newcommand{\mU}{\bm{U}}       \newcommand{\muh}{\hat{\bm{U}}}        \newcommand{\muwh}{\widehat{\bm{U}}} \newcommand{\mUt}{\tilde{\bm{U}}}        \newcommand{\muwt}{\widetilde{\bm{U}}}
\newcommand{\mv}{\bm{V}}       \newcommand{\mvh}{\hat{\bm{V}}}        \newcommand{\mvwh}{\widehat{\bm{V}}} \newcommand{\mvt}{\tilde{\bm{V}}}        \newcommand{\mvwt}{\widetilde{\bm{V}}}
\newcommand{\mw}{\bm{W}}       \newcommand{\mwh}{\hat{\bm{W}}}        \newcommand{\mwwh}{\widehat{\bm{W}}} \newcommand{\mwt}{\tilde{\bm{W}}}        \newcommand{\mwwt}{\widetilde{\bm{W}}}
\newcommand{\mx}{\bm{X}}       \newcommand{\mxh}{\hat{\bm{X}}}        \newcommand{\mxwh}{\widehat{\bm{X}}} \newcommand{\mxt}{\tilde{\bm{X}}}        \newcommand{\mxwt}{\widetilde{\bm{X}}}
\newcommand{\my}{\bm{Y}}       \newcommand{\myh}{\hat{\bm{Y}}}        \newcommand{\mywh}{\widehat{\bm{Y}}} \newcommand{\myt}{\tilde{\bm{Y}}}        \newcommand{\mywt}{\widetilde{\bm{Y}}}
\newcommand{\mz}{\bm{Z}}       \newcommand{\mzh}{\hat{\bm{Z}}}        \newcommand{\mzwh}{\widehat{\bm{Z}}} \newcommand{\mzt}{\tilde{\bm{Z}}}        \newcommand{\mzwt}{\widetilde{\bm{Z}}}


% %%%%%%%%%%%%%  TENSORS %%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\tensa}{\mathsf{A}}    \newcommand{\tensah}{\hat{\mathsf{A}}}
\newcommand{\tensb}{\mathsf{B}}    \newcommand{\tensbh}{\hat{\mathsf{B}}}
\newcommand{\tensc}{\mathsf{C}}    \newcommand{\tensch}{\hat{\mathsf{C}}}
\newcommand{\tensd}{\mathsf{D}}    \newcommand{\tensdh}{\hat{\mathsf{D}}}
\newcommand{\tense}{\mathsf{E}}    \newcommand{\tenseh}{\hat{\mathsf{E}}}
\newcommand{\tensf}{\mathsf{F}}    \newcommand{\tensfh}{\hat{\mathsf{F}}}
\newcommand{\tensg}{\mathsf{G}}    \newcommand{\tensgh}{\hat{\mathsf{G}}}
\newcommand{\tensh}{\mathsf{H}}    \newcommand{\tenshh}{\hat{\mathsf{H}}}
\newcommand{\tensi}{\mathsf{I}}    \newcommand{\tensih}{\hat{\mathsf{I}}}
\newcommand{\tensj}{\mathsf{J}}    \newcommand{\tensjh}{\hat{\mathsf{J}}}
\newcommand{\tensk}{\mathsf{K}}    \newcommand{\tenskh}{\hat{\mathsf{K}}}
\newcommand{\tensl}{\mathsf{L}}    \newcommand{\tenslh}{\hat{\mathsf{L}}}
\newcommand{\tensm}{\mathsf{M}}    \newcommand{\tensmh}{\hat{\mathsf{M}}}
\newcommand{\tensn}{\mathsf{N}}    \newcommand{\tensnh}{\hat{\mathsf{N}}}
\newcommand{\tenso}{\mathsf{O}}    \newcommand{\tensoh}{\hat{\mathsf{O}}}
\newcommand{\tensp}{\mathsf{P}}    \newcommand{\tensph}{\hat{\mathsf{P}}}
\newcommand{\tensq}{\mathsf{Q}}    \newcommand{\tensqh}{\hat{\mathsf{Q}}}
\newcommand{\tensr}{\mathsf{R}}    \newcommand{\tensrh}{\hat{\mathsf{R}}}
\newcommand{\tenss}{\mathsf{S}}    \newcommand{\tenssh}{\hat{\mathsf{S}}}
\newcommand{\tenst}{\mathsf{T}}    \newcommand{\tensth}{\hat{\mathsf{T}}}
\newcommand{\tensu}{\mathsf{U}}    \newcommand{\tensuh}{\hat{\mathsf{U}}}
\newcommand{\tensv}{\mathsf{V}}    \newcommand{\tensvh}{\hat{\mathsf{V}}}
\newcommand{\tensw}{\mathsf{W}}    \newcommand{\tenswh}{\hat{\mathsf{W}}}
\newcommand{\tensx}{\mathsf{X}}    \newcommand{\tensxh}{\hat{\mathsf{X}}}
\newcommand{\tensy}{\mathsf{Y}}    \newcommand{\tensyh}{\hat{\mathsf{Y}}}
\newcommand{\tensz}{\mathsf{Z}}    \newcommand{\tenszh}{\hat{\mathsf{Z}}}

% ==================================================== FANCY LETTERS =============================================================
\newcommand{\ac}{\mathcal{a}}    \newcommand{\Ac}{\mathcal{A}}   \newcommand{\ascr}{\mathscr{a}}    \newcommand{\Ascr}{\mathscr{A}}
\newcommand{\bc}{\mathcal{b}}    \newcommand{\Bc}{\mathcal{B}}   \newcommand{\bscr}{\mathscr{b}}    \newcommand{\Bscr}{\mathscr{B}}
\newcommand{\cc}{\mathcal{c}}    \newcommand{\Cc}{\mathcal{C}}   \newcommand{\cscr}{\mathscr{c}}    \newcommand{\Cscr}{\mathscr{C}}
\newcommand{\dc}{\mathcal{d}}    \newcommand{\Dc}{\mathcal{D}}   \newcommand{\dscr}{\mathscr{d}}    \newcommand{\Dscr}{\mathscr{D}}
\newcommand{\ec}{\mathcal{e}}    \newcommand{\Ec}{\mathcal{E}}   \newcommand{\escr}{\mathscr{e}}    \newcommand{\Escr}{\mathscr{E}}
\newcommand{\fc}{\mathcal{f}}    \newcommand{\Fc}{\mathcal{F}}   \newcommand{\fscr}{\mathscr{f}}    \newcommand{\Fscr}{\mathscr{F}}
\newcommand{\gc}{\mathcal{g}}    \newcommand{\Gc}{\mathcal{G}}   \newcommand{\gscr}{\mathscr{g}}    \newcommand{\Gscr}{\mathscr{G}}
\newcommand{\hc}{\mathcal{h}}    \newcommand{\Hc}{\mathcal{H}}   \newcommand{\hscr}{\mathscr{h}}    \newcommand{\Hscr}{\mathscr{H}}
\newcommand{\ic}{\mathcal{i}}    \newcommand{\Ic}{\mathcal{I}}   \newcommand{\iscr}{\mathscr{i}}    \newcommand{\Iscr}{\mathscr{I}}
\newcommand{\jc}{\mathcal{j}}    \newcommand{\Jc}{\mathcal{J}}   \newcommand{\jscr}{\mathscr{j}}    \newcommand{\Jscr}{\mathscr{J}}
\newcommand{\kc}{\mathcal{k}}    \newcommand{\Kc}{\mathcal{K}}   \newcommand{\kscr}{\mathscr{k}}    \newcommand{\Kscr}{\mathscr{K}}
\newcommand{\lc}{\mathcal{l}}    \newcommand{\Lc}{\mathcal{L}}   \newcommand{\lscr}{\mathscr{l}}    \newcommand{\Lscr}{\mathscr{L}}
\newcommand{\mcal}{\mathcal{m}}  \newcommand{\Mc}{\mathcal{M}}   \newcommand{\mscr}{\mathscr{m}}    \newcommand{\Mscr}{\mathscr{M}}
\newcommand{\nc}{\mathcal{n}}    \newcommand{\Nc}{\mathcal{N}}   \newcommand{\nscr}{\mathscr{n}}    \newcommand{\Nscr}{\mathscr{N}}
\newcommand{\oc}{\mathcal{o}}    \newcommand{\Oc}{\mathcal{O}}   \newcommand{\oscr}{\mathscr{o}}    \newcommand{\Oscr}{\mathscr{O}}
\newcommand{\pc}{\mathcal{p}}    \newcommand{\Pc}{\mathcal{P}}   \newcommand{\pscr}{\mathscr{p}}    \newcommand{\Pscr}{\mathscr{P}}
\newcommand{\qc}{\mathcal{q}}    \newcommand{\Qc}{\mathcal{Q}}   \newcommand{\qscr}{\mathscr{q}}    \newcommand{\Qscr}{\mathscr{Q}}
\newcommand{\rc}{\mathcal{r}}    \newcommand{\Rc}{\mathcal{R}}   \newcommand{\rscr}{\mathscr{r}}    \newcommand{\Rscr}{\mathscr{R}}
\newcommand{\scal}{\mathcal{s}}  \newcommand{\Sc}{\mathcal{S}}   \newcommand{\sscr}{\mathscr{s}}    \newcommand{\Sscr}{\mathscr{S}}
\newcommand{\tc}{\mathcal{t}}    \newcommand{\Tc}{\mathcal{T}}   \newcommand{\tscr}{\mathscr{t}}    \newcommand{\Tscr}{\mathscr{T}}
\newcommand{\uc}{\mathcal{u}}    \newcommand{\Uc}{\mathcal{U}}   \newcommand{\uscr}{\mathscr{u}}    \newcommand{\Uscr}{\mathscr{U}}
\newcommand{\vcal}{\mathcal{v}}  \newcommand{\Vc}{\mathcal{V}}   \newcommand{\vscr}{\mathscr{v}}    \newcommand{\Vscr}{\mathscr{V}}
\newcommand{\wc}{\mathcal{w}}    \newcommand{\Wc}{\mathcal{W}}   \newcommand{\wscr}{\mathscr{w}}    \newcommand{\Wscr}{\mathscr{W}}
\newcommand{\xc}{\mathcal{x}}    \newcommand{\Xc}{\mathcal{X}}   \newcommand{\xscr}{\mathscr{x}}    \newcommand{\Xscr}{\mathscr{X}}
\newcommand{\yc}{\mathcal{y}}    \newcommand{\Yc}{\mathcal{Y}}   \newcommand{\yscr}{\mathscr{y}}    \newcommand{\Yscr}{\mathscr{Y}}
\newcommand{\zc}{\mathcal{z}}    \newcommand{\Zc}{\mathcal{Z}}   \newcommand{\zscr}{\mathscr{z}}    \newcommand{\Zscr}{\mathscr{Z}}


% ================= NORMS ===========================
\newcommand{\mynorm}[2]{\| {#1} \|_{#2}}
\newcommand{\norm}[2]{\mynorm{#1}{#2}}
\newcommand{\bignorm}[2]{\left\| {#1} \right\|_{#2}}

\newcommand{\norml}[1]{\mynorm{#1}{1}}
\newcommand{\bignorml}[1]{\bignorm{#1}{1}}

\newcommand{\infnorm}[1]{\mynorm{#1}{\infty}}
\newcommand{\biginfnorm}[1]{\bignorm{#1}{\infty}}

\newcommand{\oneinf}{\ell_{1,\infty}}
\newcommand{\onetwo}{\ell_{1,2}}
\newcommand{\oneinfnorm}[1]{\mynorm{#1}{1,\infty}}
\newcommand{\bigoneinf}[1]{\bignorm{#1}{1,\infty}}

\newcommand{\onetwonorm}[1]{\mynorm{#1}{1,2}}
\newcommand{\bigonetwo}[1]{\bignorm{#1}{1,2}}

\newcommand{\enorm}[1]{\mynorm{#1}{2}}
\newcommand{\bigenorm}[1]{\bignorm{#1}{2}}

\newcommand{\znorm}[1]{\mynorm{#1}{0}}
\newcommand{\bigznorm}[1]{\bignorm{#1}{0}}

\newcommand{\frob}[1]{\|{#1}\|_{\text{F}}}
\newcommand{\bigfrob}[1]{\bignorm{#1}{\text{F}}}

\newcommand{\grpnorm}[2]{\norm{#1}{\text{Gr}(#2)}}

% ================= INTEGER FUNCTIONS ==================
\newcommand{\floor}[1]{\lfloor{#1}\rfloor}
\newcommand{\ceil}[1]{\lceil{#1}\rceil}
\newcommand{\bigfloor}[1]{\left\lfloor{#1}\right\rfloor}
\newcommand{\bigceil}[1]{\left\lceil{#1}\right\rceil}


% ================ SUMs, INTEGRALS, etc ================
\newcommand{\nlsum}{\sum\nolimits}
\newcommand{\nlprod}{\prod\nolimits}
\newcommand{\nlint}{\int\nolimits}
\newcommand{\nlmin}{\min\nolimits}


% ================ OTHER VECTOR FUNCTIONS ====================

\newcommand{\ip}[2]{\langle {#1},\, {#2} \rangle}




% =============== ANALYSIS ==========================
\newcommand{\set}[1]{\left\{ {#1}\right\}}
\newcommand{\fdel}[2]{\frac{\partial {#1}}{\partial {#2}}}
\newcommand{\sdel}[2]{{\partial {#1}}/{\partial {#2}}}


% =============== FONT RELATED =======================
\newcommand{\sml}[1]{{\small #1}}


% =============== USEFUL SETS, FIELDS, ETC. ===========================
\newcommand{\reals}{\mathbb{R}}
\newcommand{\complex}{\matbb{C}}
\newcommand{\integers}{\mathbb{Z}}
\newcommand{\posdef}[1]{\Sc_{++}^{#1}}
\newcommand{\semidef}[1]{\Sc_+^{#1}}

% =============== MISC CONSTANTS ============================
\newcommand{\half}{\tfrac{1}{2}}
\newcommand{\third}{\tfrac{1}{3}}
\newcommand{\fourth}{\tfrac{1}{4}}
\newcommand{\onehalf}{\tfrac{3}{2}}

% =================== MISC FUNCTIONS ======================
\newcommand{\fromto}[3]{\sml{$#1 \le #2 \le #3$}}
% %%%%%%%%%%% MATH KEYWORDS %%%%%%%%%%%%%%%%%%%%%%%%%%
\DeclareMathOperator*{\argmin}{argmin}
\DeclareMathOperator*{\argmax}{argmax}
\DeclareMathOperator{\dom}{dom}
\DeclareMathOperator{\interior}{int}
\DeclareMathOperator{\rank}{rank}
\DeclareMathOperator{\ri}{ri}
\DeclareMathOperator{\sgn}{sgn}
\DeclareMathOperator{\trace}{Tr}
\DeclareMathOperator{\Diag}{Diag}
\DeclareMathOperator{\range}{range}
\DeclareMathOperator{\vect}{vec}
\DeclareMathOperator{\prox}{prox}
\DeclareMathOperator{\intr}{int}
\DeclareMathOperator{\relint}{ri}
